Accurate Parameter Estimation for Risk-aware Autonomous Systems

Analysis and synthesis of safety-critical autonomous systems are carried out using models which are often dynamic. Two central features of these dynamic systems are parameters and unmodeled dynamics. This paper addresses the use of a spectral lines-based approach for estimating parameters of the dynamic model of an autonomous system. Existing literature has treated all unmodeled components of the dynamic system as sub-Gaussian noise and proposed parameter estimation using Gaussian noise-based exogenous signals. In contrast, we allow the unmodeled part to have deterministic unmodeled dynamics, which are almost always present in physical systems, in addition to sub-Gaussian noise. In addition, we propose a deterministic construction of the exogenous signal in order to carry out parameter estimation. We introduce a new tool kit which employs the theory of spectral lines, retains the stochastic setting, and leads to non-asymptotic bounds on the parameter estimation error. Unlike the existing stochastic approach, these bounds are tunable through an optimal choice of the spectrum of the exogenous signal leading to accurate parameter estimation. We also show that this estimation is robust to unmodeled dynamics, a property that is not assured by the existing approach. Finally, we show that under ideal conditions with no unmodeled dynamics, the proposed approach can ensure a $\tilde{O}(\sqrt{T})$ regret, matching existing literature. Experiments are provided to support all theoretical derivations, which show that the spectral lines-based approach outperforms the Gaussian noise-based method when unmodeled dynamics are present, in terms of both parameter estimation error and Regret obtained using the parameter estimates with a Linear Quadratic Regulator in feedback.

==> body/old/conclusions.tex <==
We develop tools for analysis of discrete-time and stochastic systems over a finite time which employs the theory of spectral lines. By providing a natural decoupling of deterministic and stochastic aspects of a signal in Definition \ref{discrete-stochastic-spectral}, we provide an appropriate definition by which tools from adaptive control can be applied to recent settings considered in the machine learning literature.

To show the efficacy of our theoretical tools, we consider two applications. The first is in estimation of linear dynamical systems subject to external random noise, as widely considered in recent literature \citep{Abbasi2011, Dean_2018a, Dean_2018, Matni2019, Sarkar_2019, Sarkar_2019a, Wagenmaker2020}. While the recent literature often selects the control input based on independent realizations of Gaussian noise, we propose a spectral lines based exogenous signal, and use a new theory of discrete stochastic spectral lines to analyze parameter estimation rates. 

The second application is in estimation of a linear dynamical system subject to both external random noise and unobserved deterministic unmodeled dynamics, which has not yet been considered in recent literature but has far reaching applications. Using the tools of spectral lines, we are again able to show appropriate estimation rates in the finite-time setting with high probability.

==> body/old/experiments.tex <==
To illustrate the efficacy of the spectral-lines based approach, we consider the system \eqref{unmodeled-intro-x}-\eqref{unmodeled-intro-w} with the following form for the linear components of the system.

\begin{align}
    A_* = \begin{bmatrix}
    0 & 1 & 0 \\
    0 & 0 & 1 \\
    a_1 & a_2 & a_3
    \end{bmatrix}, \qquad B_* = \begin{bmatrix}
    0 \\ 0 \\ 1
    \end{bmatrix} \label{eq:matrices}
\end{align}

As such, these linear components are in control canonical form \cite{Goodwin_1984, Ljung_1987}. The unmodeled dynamics are represented by the following non-linear dynamics.

\begin{align}
    w_{k} &= \begin{bmatrix} 1 & 1 & 1
    \end{bmatrix}^\top \times c \times \bar{w}_k^2, \label{eq:unmodeled-nonlin} \\ \bar{w}_k &= \alpha w_{k-1} + \alpha(u_k - \beta u_{k-1}) \,, \label{eq:unmodeled-highpass}
\end{align}

which represent a non-linear transformation of a high pass filter on the control input $u_k$. With the system defined as in \eqref{eq:matrices}-\eqref{eq:unmodeled-highpass}, we then use the following control inputs in order to estimate the system. The white noise based input , as in Sarkar and Rakhlin \cite{Sarkar_2019}, is selected as

\begin{equation}
    \label{eq:noise_input}
    u_k = s_k \qquad s_k \sim \mathcal{N}(0, E_0^2) \,,
\end{equation}

and the spectral-lines based input is selected based on a single epoch in line 5 in Algorithm \ref{alg:example}, 

\begin{equation}
    \label{eq:pe_input}
    u_k = u_{spec, k} = E_0 \sum_{i = 1}^2 \cos (2 \pi f_i t) \,.
\end{equation}

The selection of control inputs ensures $\sum_{k = 1}^T \E\left[ s_k^2 \right] = \sum_{k = 1}^T u_{spec,k}^2 = T E_0$, as to provide a comparison of signals with equivalent energy. We compare the effect of our proposed approach in \eqref{eq:pe_input} with that in \eqref{eq:noise_input} using two different metrics, (1) parameter estimation errors and (2) Regret, computed using the parameter estimates and the robust adaptive LQR of \cite{Dean_2018}. In each method, the frequencies $f_i$ are selected based on the problem setting, emulating how practitioners may select frequency content based on the application. Details and parameter selections are discussed in the Appendix.



(1) \emph{Parameter estimation errors:} Figure \ref{fig:exp-results} illustrates the estimation errors obtained using \eqref{eq:pe_input} (red) and \eqref{eq:noise_input} (blue) as a function of the input energy $E_0$. %While larger $E_0$ typically results in smaller parameter estimation rates in the setting where the unobserved disturbance is due to zero-mean noise \cite{Dean_2018, Sarkar_2019}, here we find the opposite relationship, as the unobserved deterministic disturbance increases with the magnitude of the control input. 
Notably, the spectral-lines based input has both lower estimation error and less variability in the parameter estimation error, as the spectral-lines based input does not excite the unmodeled dynamics.


\begin{figure}[!b]
    \centering
    \includegraphics[width = 0.8\textwidth]{imgs/wn_sin_diff.png}
    \caption{Estimation errors for the system \eqref{eq:matrices}-\eqref{eq:unmodeled-highpass}, for various levels $E_0$ of energy of input signals. Frequencies for the spectral-lines based input are $f_1 = 0.05$ and $f_2 = 0.3$ based on Line 10 of Algorithm 1. Experiments are run $100$ times, for $T = 500$. Error bars correspond to one standard deviation.}
    \label{fig:exp-results}
\end{figure}


(2) \emph{Regret:} We compute a control input $u_k$ and an LQR gain $K^{(i)}$ as outlined in Algorithm \ref{alg:example} in Lines 5 and 8 in Dean et al. \cite{Dean_2018}, and Regret $(T)$ defined as in Section 2 of Dean et al. \cite{Dean_2018}. Figure \ref{fig:regret-results} shows the Regret in orange for the input as in \eqref{eq:noise_input}, where $\eta_k$ in line 5 of Algorithm \ref{alg:example} in Dean et al. \cite{Dean_2018} is chosen as $s_k$ in \eqref{eq:noise_input}. The corresponding Regret when the same $\eta_k$ in Dean et al. \cite{Dean_2018} is chosen as $u_{spec,k}$ in \eqref{eq:pe_input} is shown in green in the same figure, both as a function of the iteration $i$. These performances are benchmarked against an `optimal' controller $u_k = K_* x_k$, where $K_*$ is the solution to the discrete algebraic Riccati solution when $A_*$ and $B_*$ are known. In both figures, the parameters in \eqref{eq:unmodeled-nonlin}-\eqref{eq:unmodeled-highpass} are chosen so that unmodeled dynamics is 0.1 times the modeled part at low frequencies. In the top figure, the noise level is 0.01 times the signal, typical in practical applications \cite[Chapter 6.2.1]{Lavretsky2013}, while in the bottom figure, the noise to signal ratio is 0.1. In both cases, our approach outperforms the noise-based procedure.



\begin{figure}[!t]
    \centering
    \includegraphics[trim=0 0 0 10, width = 0.8\textwidth]{imgs/old/regret_hundredth.png}
    \includegraphics[trim=0 10 0 0, width = 0.8\textwidth]{imgs/old/regret_larger.png}
    
    \caption{Median and 90th percentile of Regret over time, at two levels of external noise. In both cases, the spectral-lines based exploration, with $f_1 = 0.03$ and $f_2 = 0.05$, outperforms the white noise-based exploration.}
    \label{fig:regret-results}
\end{figure}

==> body/old/lti-estimation.tex <==
In this section, we consider the system in \eqref{lti-noisy-intro}
and will provide a new analysis for estimation of $A_* \in \R^{n \times n}$ and $B_* \in \R^{n \times m}$ given the choice of a \emph{deterministic} $u_k$ and observations $x_k$. The transfer function from $u_k$ to $\phi_k = [x_k^\top u_k^\top]^\top$ may be written as
\begin{align*}
 \boldphi (e^{j\omega}) = \begin{bmatrix}(e^{j\omega} I - A_*)^{-1} B_* \\
I_{m}\end{bmatrix} \u(e^{j\omega}) ~~+ \\
\begin{bmatrix}
(e^{j\omega}I - A_*)^{-1}  \\
0
\end{bmatrix} \boldeta(e^{j\omega}) \,. 
\end{align*}
Hence, if $u_k$ has a sub-Gaussian spectral line from $0$ to $T-1$ at frequency $\omega_0$, with radius $0$ and amplitude $\bar{u}(\omega_0)$, it follows from Lemma \ref{spectral-transfer} that $\phi_k$ has a sub-Gaussian spectral line from $0$ to $T-1$ at frequency $\omega_0$ with finite radius and amplitude \[ \bar{\phi}(\omega_0) = \begin{bmatrix}(e^{j \omega}I - A_*)^{-1} B_* \\ I_m \end{bmatrix}  \bar{u}(\omega_0) \,,\] 
as long as $\omega_0 \in \Omega_T$. 
With the expected information matrix of the regressor of system \eqref{lti-noisy-intro} defined, we now present the first main contribution of this work.
\begin{theorem}
\label{system-id-thm}
Consider the dynamical system in \eqref{lti-noisy-intro}, with expected information matrix $\bar{\Phi}$ as in Definition \ref{big-phi} for $\phi_k = [x_k^\top u_k^\top]^\top$. Let $(\hat{A}, \hat{B})$ be the least-squares estimates of $A_*$ and $B_*$,
\begin{equation} \label{least-squares}
    (\hat{A}, \hat{B}) = \argmin_{A \in \R^{n\times n}, B \in \R^{n \times m}} \sum_{k = 0}^{T-1} \norm{x_{k+1} - Ax_k - Bu_k}_2^2 \,.
\end{equation} 
If the control input $u_k$ is selected such that $\phi_k$ has $n + m$ spectral lines with linearly independent amplitudes and finite radii, then
\[
    \max \left\lbrace ||\hat{A} - A_*||, || \hat{B} - B_*|| \right\rbrace \leq \tilde{O} \left( \sqrt{\frac{1}{T \norm{\bar{\Phi}^{-1}}^{-2}}} \right)\,,
\]
with probability at least $1 - \delta$, where the $\tilde{O}$ notation discards constant and logarithmic terms.
\end{theorem}
Details of the proof of Theorem \ref{system-id-thm} may be found in Appendix \ref{a:si-proof}. We note this contribution is akin to the concentration inequalities developed in \cite{Simchowitz_2018, Sarkar_2019}.

Theorem \ref{system-id-thm} shows that the choice of deterministic exogenous signal matters in the context of system estimation. The estimation rate of the least-squares estimate of $A_*$ and $B_*$ will depend on the spectral content of the exogenous input $\{u_k\}_{k=0}^{T-1}$. While the relationship between parameter identification and spectrum of input data is well known in the machine learning community \cite{Bishop2006, Vershynin2019}, it is worth stating here that our framework provides a condition based on spectral lines by which a practitioner can achieve well-conditioned data in practice. In particular, the practitioner can achieve such well-conditioning by selecting an exogenous input with $n + m$ spectral lines, and our upper bound on estimation error can be optimized as outlined in Line 6 of Algorithm \ref{alg:least_squares}. As mentioned before, any further constraints on the exogenous signal may be incorporated in Line 6 as well.

==> body/old/unmodeled.tex <==
In this section, we now consider the system \eqref{unmodeled-intro-x}-\eqref{unmodeled-intro-w}, where the influence of the spectrum of $u_k$ on $x_k$ is more complex due to the presence of unmodeled dynamics $w_k$. By exploiting the structure of \eqref{unmodeled-intro-x}-\eqref{unmodeled-intro-w}, we may rewrite the system in the frequency domain as
\begin{equation} \label{unmodeled-freq-domain}
\begin{aligned}
    \x(e^{j \omega}) &= (e^{j \omega}I - A_*)^{-1}B_* \u(e^{j \omega}) + \\&\quad (e^{j \omega}I - A_*)^{-1} \bigg(\w(e^{j \omega}) + \boldeta(e^{j \omega}) \bigg)\,.
\end{aligned}
\end{equation}
In order for the above statement to hold, we make the following technical assumption.
\begin{assumption} \label{wk-assumption}
In the system \eqref{unmodeled-intro-x}-\eqref{unmodeled-intro-w}, $f$ is Lipschitz \citep{Rudin1987}. %, i.e. for any deterministic and bounded choice of $\{u_k\}_{k=0}^{T-1}$, the sequence $\{w_k\}_{k=0}^{T-1}$ is deterministic and bounded.
\end{assumption}
In particular, Assumption \ref{wk-assumption} implies that, as long as $\{u_k\}_{k=0}^{T-1}$ is Fourier integrable in the discrete setting, then so is $\{w_k\}_{k=0}^{T-1}$ \citep{Oppenheim1999}. Under this condition, we see from \eqref{unmodeled-freq-domain} and Lemma \ref{spectral-transfer}, for $\phi_k = [x_k^\top u_k^\top]^\top$, the sequence $\{\phi_k\}_{k=0}^{T-1}$ has a spectral line at frequency $\omega_0$ from $0$ to $T - 1$ with amplitude 
\begin{align*}
    \bar{\phi}(\omega_0) = \begin{bmatrix}(e^{j \omega}I - A_*)^{-1} B_* \\ I_m \end{bmatrix} \bar{u}(\omega_0) ~~+ \\ \begin{bmatrix}
(e^{j\omega}I - A_*)^{-1}  \\
0
\end{bmatrix} \bar{w}(\omega_0) \,, 
\end{align*} 
and finite radius. Hence, the information matrix for the system is clearly defined, leading to the following result.
\begin{theorem} \label{unmodeled-estimation}
Consider the system \eqref{unmodeled-intro-x}-\eqref{unmodeled-intro-w} under Assumption \ref{wk-assumption}, and suppose the input $u_k$ is selected such that, with probability at least $1 - \delta$, 
\begin{equation} \sum_{k = 0}^{T-1} \norm{w_k} \leq m_T \,, \label{th3_condn}\end{equation}
where $m_T$ is finite. If the control input $u_k$ is selected such that $\phi_k = [x_k^\top u_k^\top]^\top$ has $n + m$ spectral lines with linearly independent amplitudes and finite radii, then the estimates $(\hat{A}, \hat{B})$ as defined in \eqref{least-squares} will satisfy, with probability at least $1 - 2 \delta$, 
\begin{align*}
     &\max \left\lbrace \norm{\hat{A} - A_*}, \norm{ \hat{B} - B_*}\right\rbrace \leq \\ 
     &\qquad\qquad\tilde{O} \left( (1 + m_T^2) \sqrt{\frac{1}{T \norm{\bar{\Phi}^{-1}}^{-2}}} \right) \,.
\end{align*}
\end{theorem}
A proof of Theorem \ref{unmodeled-estimation} can be found in Appendix \ref{a:unmodeled-proof}. In order to show the utility of Theorem \ref{unmodeled-estimation}, we must consider the form of the quantity $m_T$, which the practitioner would wish to minimize. This quantity may not necessarily be small for all choices of $f(\cdot)$ or arbitrary selections of $u_k$. However, $m_T$ can be shown to be of small order in the following two common settings. Clearly more research is needed to relax the condition in \eqref{th3_condn} to increase the scope of applicability of the proposed approach. %, showing that Theorem \ref{unmodeled-estimation} provides a useful parameter estimation bound.


\begin{example}[High Pass Filter]
Suppose the operator $f(\cdot)$ in \eqref{unmodeled-intro-w} is such that
\begin{equation} \label{2ndeqn-example1}
w_{k} = \sum_{i=1}^n a_i w_{k-i} + \sum_{i=1}^m b_i u_{k-i}
\end{equation}
and $a_i,b_j$ are such that the transfer function from $u_k$ to $w_k$ is a high-pass filter. Then, a proper choice of $\Omega$ as noted in Definition \ref{big-phi} will ensure that $w_k$ will tend to zero exponentially with $k$ \citep{Goodwin_1984}, which will imply in turn that $m_T=O(1)$.
\end{example}

\begin{example}[Small Non-Linearities] \label{small-nonlinearity}
Suppose \eqref{unmodeled-intro-w} is such that
\begin{equation} \label{eq2}
\begin{aligned}
\overline w_{k} &= \sum_{i=1}^n a_i w_{k-i} + \sum_{i=1}^m b_i u_{k-i}\\
w_k&=f(\overline w_k) \,.
\end{aligned}
\end{equation}
If the function $f(\cdot)$ is such that the choice of $u_k$ will guarantee $\norm{w_k} = O(1/k^{1 + \epsilon})$ for any $\epsilon > 0$, then it implies that $m_T = O(1)$. This can occur, for example, if $f(\cdot)$ corresponds to higher-order terms, and $u_k$ and initial conditions $w_0$ and $x_0$ are sufficiently small \citep{Khalil2002}.
\end{example}
